The Redshift of GRB 190829A/ SN 2019oyw: A Case Study of GRB-SN Evolution

The nearby long gamma-ray burst (GRB) 190829A was observed using the HST/WFC3/IR grisms about four weeks to 500 days after the burst. We find the spectral features of its associated supernova, SN 2019oyw, are redshifted by several thousands km/s compared to the redshift of the large spiral galaxy on which it is superposed. This velocity offset is seen in several features but most clearly in Ca II NIR triplet $\lambda\lambda$ 8498, 8542, 8662 (CaIR3). We also analyze VLT/FORS and X-shooter spectra of the SN and find strong evolution with time of its P-Cygni features of CaIR3 from the blue to the red. However, comparison with a large sample of Type Ic-BL and Ic SNe shows no other object with the CaIR3 line as red as that of SN 2019oyw were it at the z = 0.0785 redshift of the disk galaxy. This implies that SN 2019oyw is either a highly unusual SN or is moving rapidly with respect to its apparent host. Indeed, using CaIR3 we find the redshift of SN 2019oyw is 0.0944 <= z <= 0.1156. The GRB-SN is superposed on a particularly dusty region of the massive spiral galaxy; therefore, while we see no sign of a small host galaxy behind the spiral, it could be obscured. Our work provides a surprising result on the origins of GRB 190829A, as well as insights into the time evolution of GRB-SNe spectra and a method for directly determining the redshift of a GRB-SN using the evolution of strong spectral features such as CaIR3.

==> DOI_number.tex <==
DOI: 10.17909/yz9m-xb66


==> tableXS.tex <==
\begin{deluxetable*}{clhllc}
\tablenum{1.2}
\tablecaption{Datasets from ground-based facilities \label{table:xs}}
\tablewidth{0pt}
\tablehead{
\colhead{Proposal ID} & \colhead{Epoch} & \nocolhead{MJD} & \colhead{Instrument} & \colhead{Filter} &
\colhead{Total Exposure (s)}
}
\decimalcolnumbers
\startdata
??? & 2019-09-23 & - & $XS$ & ??? & ??? \\
??? & 2021-11-12 & - & $XS$ & ??? & ??? \\
\enddata
\end{deluxetable*}

